DriveThru: a Document Extraction Platform and Benchmark Datasets for Indonesian Local Language Archives

Indonesia is one of the most diverse countries linguistically. However, despite this linguistic diversity, Indonesian languages remain underrepresented in Natural Language Processing (NLP) research and technologies. In the past two years, several efforts have been conducted to construct NLP resources for Indonesian languages. However, most of these efforts have been focused on creating manual resources thus difficult to scale to more languages. Although many Indonesian languages do not have a web presence, locally there are resources that document these languages well in printed forms such as books, magazines, and newspapers. Digitizing these existing resources will enable scaling of Indonesian language resource construction to many more languages. In this paper, we propose an alternative method of creating datasets by digitizing documents, which have not previously been used to build digital language resources in Indonesia. DriveThru is a platform for extracting document content utilizing Optical Character Recognition (OCR) techniques in its system to provide language resource building with less manual effort and cost. This paper also studies the utility of current state-of-the-art LLM for post-OCR correction to show the capability of increasing the character accuracy rate (CAR) and word accuracy rate (WAR) compared to off-the-shelf OCR.

==> sections/05-future-directions.tex <==
\section{Future Directions}

% DriveThru will be the baseline of our data-collecting platform following \cite{CURL_Körner_Helfer_Schröder_Eckart_Goldhahn} data-collecting ideas. Rather than inputting url entry, broaden language resource collection methods.

In this work, we only focused on building the document extraction tools for further language resource collecting and dataset-making, we also shared our benchmark dataset for some local language resources as the proof of concept of our works. In the next phase, we are going to broaden our language variety by putting other language resources we found throughout the time.

As the project is in the form of a web application, there must be another improvement and adding features to improve the system capability as well as the user accessibility, even though it is designed as user-friendly as possible we will \textit{not close our mind} \textit{(use another term) }if there were another best practices on user experience application design.

% Since it does not cost much effort, we plan to add manual correction features on DriveThru apps, So users not only upload their data, waiting the data to be processed, and preview the data, but can further do something with their data afterward.

% For the continuity of the project, since it is developed by the academic institution there are no blocked ways.



% #################################################




% There are several key areas where the system can be further enhanced to escalate its overall functionality and accessibility. 

% We're doing it right now, so it won't count as future directions anymore. But I keep this sections as a highlight.
% Firstly, we plan to refine the OCR model to achieve higher accuracy and cleaner results %. By refining the model, it is possible to achieve more accurate and cleaner results 
% when digitizing printed language resources. This improvement combined with better pre-processing of the resulting text would contribute to the overall quality and reliability of the uploaded datasets. In the pipeline is also the plan to add language identification features and improvement of the OCR results for low resource languages based on existing language resources such as dictionaries for these languages. 

% Points need to be explained
% \begin{itemize}
%     \item Keberlangsungan proyek ini ke depannya (continuity), siapa yang membiayai, siapa yang melanjutkan development, dll.
%     \item data availability, where the data will be shared?
% \end{itemize}

% ####################################### OLD ######################################


% Speech-to-text 
% Secondly, to expand the system's capabilities as well as for the inclusion of languages that do not have written forms, %As part of expanding the system's capabilities, 
% one of the future enhancements we plan to add is the ability to collect data in audio form by partnering with platforms that provide speech data collection through various channels (phones, smartphones, internet) such as Paroli\footnote{\href{https://caritas.paroli.live/welcome}{https://caritas.paroli.live/welcome}}. 
% By collecting speech language data and adding features for users who are native speakers to contribute to transcribing these speech data, we can further scale language resource collection and preserve linguistic diversity even for lesser-known languages. 

% Gamification features plan
% Thirdly, to enhance user engagement and encourage continuous contributions, we plan to introduce gamification features \cite{RAJAN2020100299}. Users will be encouraged to contribute their language materials regularly with features like tracking their daily contributions and earning points as rewards. This gamified approach will not only motivate users to consistently participate in uploading language resources but also make the platform more enjoyable and engaging. Furthermore, we plan to implement location-based events, seasonal challenges, as well a payment reward system to incentivize contributions. %as part of the gamification strategy. 
% By focusing on specific regions or periods, we can have the opportunity to prioritize languages that might have limited resources. These gamified features will not only make the platform more enjoyable but also foster a sense of accomplishment and community involvement in preserving and enriching linguistic diversity.

% Community building plan
% Lastly, by involving everyone in the Indonesian language community, this research initiative holds the potential to serve as a social movement for language preservation. We plan to engage and work with individuals and communities %with shared interests %, not limited to computer science backgrounds in specific universities but 
% including diverse groups from various language communities, universities, as well as organizations that work with many communities in remote parts of the country such as the Indonesian Red Cross. Additionally, we plan to conduct extensive campaigns through social media, mainstream media, and other channels to raise awareness of our platform RagamBahasa. To facilitate effective communication and collaboration among contributors, we also plan to utilize  online communication platforms like Slack or Discord. 

==> sections/tablesa.tex <==

% % % % % % % % % % %
% Data sources        %
% % % % % % % % % % %

\begin{table*}[h]
\centering
\begin{tabular}{@{}rlllll@{}}
\toprule
\multicolumn{1}{l}{\textbf{\#}} & \textbf{Language} & \textbf{ISO} & \textbf{Source Title}                             & \textbf{Genre} & \multicolumn{1}{l}{\textbf{\makecell[l]{Total of\\Image}}} \\ \midrule
1                               & Balinese          & ban          & I Bagus Caratan                                   & Children       & 26                                          \\
2                               & Balinese          & ban          & Leak Pemoroan                                     & Short Story    & 24                                          \\
3                               & Balinese          & ban          & \makecell[l]{Ejaan Bahasa Daerah Bali\\yang Disempurnakan 1974}& Learning Book  & 13                                          \\
4                               & Balinese          & ban          & Majalah Suara Saking Bali Edisi VII               & Magazine       & 12                                          \\
5                               & Balinese          & ban          & Paparikan Lawe                                    & Learning Book  & 10                                          \\
6                               & Balinese          & ban          & \makecell[l]{Pedoman Umum Ejaan Bahasa Bali\\Dengan Huruf Latin}& Learning Book  & 15                                          \\
7                               & Javanese          & jav          & Panjebar Semangat                                 & Magazine       & 100                                         \\
8                               & Sundanese         & sun          & Carita ti Carita                                  & Short story    & 5                                           \\
9                               & Sundanese         & sun          & Hayam Gecok Ngeunah                               & Short story    & 5                                           \\
10                              & Sundanese         & sun          & Mangle                                            & Magazine       & 25                                          \\
 11& Sundanese& sun& Wawacan Rengganis & Story Book  &16\\
 12& Sundanese& sun& Wawacan Sejarah Anbia & Story book  &10\\
 13& Sundanese& sun& Raja Neger Jeung Bangsa Arab & Story book  &17\\
 14& Sundanese& sun& Lain Eta & Story book  &12\\
 15& Sundanese& sun& Istri kasasar & Story book  &10\\
16& Minangkabau       & min          & \makecell[l]{Kaba Bujang Paman\\Dan Kaba Rambun Pamenan}         & Novel          & 55                                          \\
17& Minangkabau       & min          & \makecell[l]{Kaba Kambang Luari Sutan\\Pangaduan}                & Novel          & 45                                          \\
\midrule
\multicolumn{5}{c}{\textbf{Total}}                                                                                                      & \textbf{400}\\ \bottomrule
\end{tabular}
\caption{A list of document titles from four different languages with their respective genres. We collected 335 images from a total of 12 books spanning various genres in language resource archives to use for benchmark datasets.}
\label{tab:dataset}
\end{table*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
    \centering
    \begin{tabular}{|m{0.18\textwidth}|m{0.22\textwidth}|m{0.22\textwidth}|m{0.22\textwidth}|}
        \hline
        \textbf{Image} & \textbf{OCR Output} & \textbf{Human Annotation} & \textbf{Post-OCR Correction} \\
        \hline
        \includegraphics[width=0.2\textwidth]{figures/ocr-res/47.png} & 
        Sing unik maneh, Bekecot pranyata ndu- weni untu kang uakeehhh banget lo. Adhik- adhik ngerti pira jumlahe? Pranyata untune Bekecot ana 14.175. Untu iki cilik-cilik ba- nget lan wujude kaya parut. Untu iki bisa ma- mah gegodhongan kang akeh banget jroning sewengi. : : & 
        Sing unik maneh, Bekecot pranyata ndu- weni untu kang akeh banget lo. Adhik- adhik ngerti pira jumlahé? Pranyata untune Bekecot ana 14.175. Untu iki cilik-cilik ba- nget lan wujude kaya parut. Untu iki bisa ma- mah gegodhongan kang akeh banget jroning sewengi. & 
        Sing unik maneh, Bekicot pranyata nduweni untu kang uakeh banget lo. Adhik-adhik ngerti pira jumlahe? Pranyata untune Bekicot ana 14.175. Untu iki cilik-cilik banget lan wujude kaya parut. Untu iki bisa mah gegodhongan kang akeh banget jroning sewengi. \\
        \hline
        \includegraphics[width=0.18\textwidth]{figures/ocr-res/3.png} & 
        Bataan ceeiaalteleea Saati: St meinen, ~ aa Terekel Salim naek kena kai, rak ngadon sare. Teu wanieun sare di handap, sieun disampeurkeun sato galak, didodoho eukeur sare.& 
        Terekel Salim nack kena kai, rak neadon sare. Teu wanieun sare di handap, sieun disampeurkeun sato galak, didodoho eukeur& 
        Terekel Salim naek kena kai, rak ngadon sare. Teu wanieun sare di handap, sieun disampeurkeun sato galak, didodoho eukeur sare. \\
        \hline
        \includegraphics[width=0.18\textwidth]{figures/ocr-res/93.png} & 
        . eRe ; Naskah Supersemar jing tangane Pak Harto we & 
        Naskah Supersemar ing tangane Pak Harto & 
        Naskah Supersemar ing tangane Pak Harto. \\
        \hline
        \includegraphics[width=0.18\textwidth]{figures/ocr-res/92.png} & 
        tn anit ORI ETS .2.Rtee Deira ty cATE SS PEA LIA AROS TA TOS Bie > 2\% NB fe ? 4 oh ry fr any, ct sted ered Sue, ek Acnta, Fil ee na) al Ne la eet tO tee a! aD OP TI PE HOOT Eas & 
        Pangudarasa & 
        Anit ORI ETS. 2. Rtee Deira ty cATE SS PEA LIA AROS TA TOS Bie > 2\% NB fe? 4 oh ry fr any, ct sted ered Sue, ek Acnta, Fil ee na) al Ne la eet tO tee a! aD OP TI PE HOOT Eas. \\
        \hline
    \end{tabular}
    \caption{Comparison of OCR Output, Human Annotation, and Post-OCR Correction with Few-Shot Approach in GPT-4o }
\label{tab:ocr_comparison}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % % % % % % % % % %
% Number of words        %
% % % % % % % % % % %

% \begin{table*}[]
% \centering
% \begin{tabular}{@{}rlrrrrr@{}} \midrule
% \multicolumn{1}{c}{\textbf{\#}} & \textbf{Language} & \multicolumn{1}{c}{\textbf{GT}} & \multicolumn{1}{c}{\textbf{OTS}} & \multicolumn{1}{c}{\textbf{Llama3}} & \multicolumn{1}{c}{\textbf{Aya23}} & \multicolumn{1}{c}{\textbf{Cendol}} \\
% \midrule
% 1                               & Balinese          & 16138& 16207
% & & & \\
% 2                               & Javanese          & 12300& 14471
% & & & \\
% 3                               & Sundanese         & 18558& 18771
% & & & \\
% 4                               & Minangkabau       & 30368& 30614& & & \\
% \midrule
% \multicolumn{2}{c}{\textbf{Total}}                           & \multicolumn{1}{l}{77364}            & \multicolumn{1}{l}{80063}             & \multicolumn{1}{l}{}                & \multicolumn{1}{l}{}               & \multicolumn{1}{l}{}                \\ 
% \bottomrule
% \end{tabular}
% \caption{Number of tokens retrieved from Indonesian local language archives extraction, with (Llama3, Aya23, Cendol) and without (OTS) additional post-correction steps.}
% \label{tab:maxlen-eval}
% \end{table*}


\begin{table*}[h]
\centering
\begin{tabular}{@{}lcrrr@{}}
\toprule
                       & \multicolumn{4}{c}{\textbf{Languages}}                                                                                                                                \\ \midrule
\multicolumn{1}{l}{} & \multicolumn{1}{c}{\textbf{Balinese}} & \multicolumn{1}{c}{\textbf{Javanese}} & \multicolumn{1}{c}{\textbf{Sundanese}} & \multicolumn{1}{c}{\textbf{Minangkabau}} \\ \midrule
\textbf{GT}                     & \multicolumn{1}{r}{16138}                & 12300& 18558& 30368\\
\midrule
\textbf{OTS}                    & \multicolumn{1}{r}{16207}                & 14471& 18771& 30614\\ 
\textbf{Llama3 (FS)}            & \multicolumn{1}{r}{15955}                & 12897& 18524&30490\\
\textbf{Llama3 (ZS)}            & \multicolumn{1}{r}{16034}                & 11979& 18513&30389\\
\textbf{GPT-4 (FS)}             & \multicolumn{1}{r}{16010}                & 13775& 18641&30232\\
\textbf{GPT-4 (FS)}             & \multicolumn{1}{r}{15941}                & 13123& 18606&29785\\
\bottomrule
\end{tabular}
\caption{Number of tokens retrieved from Indonesian local language archives extraction, comparing between the number of ground-truth (GT), off-the-shelf (OTS) TesseractOCR, Llama3 and GPT-4 both with Few-shot (FS) and Zero-shot (ZS), respectively.}
\label{tab:maxlen-eval}
\end{table*}

% % % % % % % % % % %
% Error rate scores         %
% % % % % % % % % % %

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\vspace{-100}
\begin{table*}[]
\centering
\begin{tabular}{@{}rlrrrrr@{}}
\toprule
\multicolumn{1}{l}{} &                   & \multicolumn{5}{c}{\textbf{CAR}}                                                                                                                                                                           \\ \midrule
\multicolumn{1}{l}{} & \textbf{Language} & \multicolumn{1}{c}{\textbf{OTS}} & \multicolumn{1}{c}{\textbf{Llama3 (ZS)}} & \multicolumn{1}{c}{\textbf{Llama3 (FS)}} & \multicolumn{1}{c}{\textbf{GPT-4 (ZS)}} & \multicolumn{1}{c}{\textbf{GPT-4 (FS)}} \\
\midrule
1                    & Balinese          & 0.943                            & 0.917                                    & 0.919                                    & 0.893                                   & 0.914                                   \\
2                    & Javanese          & -0.993                           & 0.970                                    & 0.956                                    & 0.965                                   & 0.965                                   \\
3                    & Sundanese         & 0.911                            & 0.738                                    & 0.168                                    & -0.368                                  & -0.699                                  \\
4                    & Minangkabau       & 0.958                            & 0.942                                    & 0.942                                    & 0.924                                   & 0.926                                   \\
\midrule
\multicolumn{2}{c}{\textbf{avg (\%)}}    & 0.45475                          & \textbf{0.892}& 0.746                                    & 0.603                                   & 0.526                                   \\ \bottomrule
\end{tabular}
\caption{Percentage of Character Accuracy Rates (CAR) on different extraction techniques. The off-the-shelf (OTS) column means there are no additional steps to repair the extracted text, while the others perform additional post-correction steps involving LLMs. Overall, Llama3 with a Zero-shot approach outperforms other LLMs in post-correction OCR.}
\label{tab:car-eval}
\vspace{-10mm}
\end{table*}


\begin{table*}[]
\centering
\begin{tabular}{@{}rlrrrrr@{}}
\toprule
\multicolumn{1}{l}{} &                   & \multicolumn{5}{c}{\textbf{WAR}}                                                                                                                                                                           \\ \midrule
\multicolumn{1}{l}{} & \textbf{Language} & \multicolumn{1}{c}{\textbf{OTS}} & \multicolumn{1}{c}{\textbf{Llama3 (ZS)}} & \multicolumn{1}{c}{\textbf{Llama3 (FS)}} & \multicolumn{1}{c}{\textbf{GPT-4 (ZS)}} & \multicolumn{1}{c}{\textbf{GPT-4 (FS)}} \\
\midrule
1                    & Balinese          & 0.777                            & 0.808                                    & 0.818                                    & 0.795                                   & 0.757                                   \\
2                    & Javanese          & -4.04                            & 0.532                                    & -0.966                                   & -2.080                                  & -3.012                                  \\
3                    & Sundanese         & 0.777                            & 0.903                                    & 0.872                                    & 0.760                                   & 0.787                                   \\
4                    & Minangkabau       & 0.866                            & 0.806                                    & 0.779                                    & 0.879                                   & 0.879                                   \\
\midrule
\multicolumn{2}{c}{\textbf{avg (\%)}}    & -0.405                           & \textbf{0.762}& 0.375                                    & 0.088                                   & -0.147                                  \\ \bottomrule
\end{tabular}
\caption{Percentage of Word Accuracy Rates (WAR) on different extraction techniques. The off-the-shelf (OTS) column means there are no additional steps to repair the extracted text, while the others perform additional post-correction steps involving LLMs. Overall, Llama3 with a Zero-shot approach performs well compared to the other LLM in all languages.}
\label{tab:war-eval}
\end{table*}



% \begin{table*}[]
% \centering
% \begin{tabular}{@{}rlrrrrrrrr@{}}
% \toprule
% \multicolumn{1}{l}{}            &                   &\multicolumn{4}{c}{\textbf{CAR}}&\multicolumn{4}{c}{\textbf{WAR}}\\ \midrule
% \multicolumn{1}{c}{\textbf{\#}} & \textbf{Language}  & \multicolumn{1}{c}{\textbf{OTS}} & \multicolumn{1}{c}{\textbf{Llama3}} & \multicolumn{1}{c}{\textbf{Aya23}} & \multicolumn{1}{c}{\textbf{Cendol}}  & \multicolumn{1|}{c}{\textbf{OTS}} & \multicolumn{1}{c}{\textbf{Llama3}} & \multicolumn{1}{c}{\textbf{Aya23}} & \multicolumn{1}{c}{\textbf{Cendol}} \\
% \midrule
% 1                               & Balinese          & 0.943& 0.942& -0.523& -0.260& 0.777& 0.808& -0.310& -0.264\\
% \midrule
% 2                               & Javanese          & -0.993& \textbf{0.738}& -1.802& -2.626& -4.040& \textbf{0.532}& -4.819& -3.328\\
% \midrule
% 3                               & Sundanese         & 0.911& 0.917& 0.190& -0.069& 0.777& 0.806& 0.188& -0.258\\
% \midrule
% 4                               & Minangkabau       & 0.958& 0.970& 0.187& 0.236& 0.866& 0.903& 0.154& 0.043\\
% \midrule
% \multicolumn{2}{c}{\textbf{avg (\%)}}               & 0.455& \textbf{0.892}& -0.712& -0.985& -0.405& \textbf{0.762}& -1.647& -1.283\\ 
% \bottomrule
% \end{tabular}
% \caption{Percentage of Character Accuracy Rates (CAR) and Word Accuracy Rates (WAR) on different extraction techniques. The off-the-shelf (OTS) column means there are no additional steps to repair the extracted text, while the others perform additional post-correction steps involving LLMs.}
% \label{tab:cer-wer-eval}
% \end{table*}

